Sparse image reconstruction for molecular imaging

The application that motivates this paper is molecular imaging at the atomic level. When discretized at sub-atomic distances, the volume is inherently sparse. Noiseless measurements from an imaging technology can be modeled by convolution of the image with the system point spread function (psf). Such is the case with magnetic resonance force microscopy (MRFM), an emerging technology where imaging of an individual tobacco mosaic virus was recently demonstrated with nanometer resolution. We also consider additive white Gaussian noise (AWGN) in the measurements. Many prior works of sparse estimators have focused on the case when H has low coherence; however, the system matrix H in our application is the convolution matrix for the system psf. A typical convolution matrix has high coherence. The paper therefore does not assume a low coherence H. A discrete-continuous form of the Laplacian and atom at zero (LAZE) p.d.f. used by Johnstone and Silverman is formulated, and two sparse estimators derived by maximizing the joint p.d.f. of the observation and image conditioned on the hyperparameters. A thresholding rule that generalizes the hard and soft thresholding rule appears in the course of the derivation. This so-called hybrid thresholding rule, when used in the iterative thresholding framework, gives rise to the hybrid estimator, a generalization of the lasso. Unbiased estimates of the hyperparameters for the lasso and hybrid estimator are obtained via Stein's unbiased risk estimate (SURE). A numerical study with a Gaussian psf and two sparse images shows that the hybrid estimator outperforms the lasso.

==> Makefile <==

include $(HOME)/work/mrfm/papers/dtdet/global_opts.mk

.PHONY: create_dep_files create_dep_dirs d7_manuscript d7_double numbers clean 

.DEFAULT_GOAL := d7_double

DEP_FILES = ../ieee/IEEEtran.cls \
	../ieee/IEEEtran.bst \
	../ieee/IEEEabrv.bib \
	../d4/mike_lib.bib \
	$(HOME)/work/thesis/mike_thesis.bib \
	$(HOME)/work/thesis/xfig/hybrid_thres.pstex \
	$(HOME)/work/thesis/xfig/hybrid_thres.pstex_t \
	$(HOME)/work/thesis/xfig/ct_stat.pstex \
	$(HOME)/work/thesis/xfig/ct_stat.pstex_t \
	$(HOME)/work/thesis/xfig/ebd_block_diag.pstex \
	$(HOME)/work/thesis/xfig/ebd_block_diag.pstex_t \
	$(HOME)/work/thesis/xfig/em_sep_c.pstex \
	$(HOME)/work/thesis/xfig/em_sep_c.pstex_t \
	$(HOME)/work/thesis/xfig/design_pen.pstex \
	$(HOME)/work/thesis/xfig/design_pen.pstex_t \
	$(HOME)/work/thesis/xfig/sparse_model.pstex \
	$(HOME)/work/thesis/xfig/sparse_model.pstex_t

DEP_DIRS = $(HOME)/work/f05/icip06/binary/s1/snr2/t10 \
		   $(HOME)/work/f05/icip06/binary/s1/snr10/t11 \
		   $(HOME)/work/f05/icip06/js/s1/snr10/t12 \
		   $(HOME)/work/thesis/sim \
		   $(HOME)/work/f05/icip06/binary/s1/tip07 \
		   $(HOME)/work/f05/icip06/js/s1/tip_hyp07 \
		   $(HOME)/work/f05/threed

d7_manuscript: create_dep_files create_dep_dirs d7_manuscript.tex
	@echo "   .............................................."
	@echo "   ---| Running default target d7_manuscript |---"
	@echo "   ##############################################"
	@$(TEX) $@
	@echo "   ........................"
	@echo "   ---| Running $(BIB) |---"
	@echo "   ########################"
	@$(BIB) $@
	@echo "   ............................."
	@echo "   ---| Running final $(TEX) |---"
	@echo "   #############################"
	@$(TEX) $@
	@echo "   ......................."
	@echo "   ---| Running $(DVIPS) |---"
	@echo "   #######################"
	$(DVIPS) $(DVIPS_OPTS) < $@.dvi > $@.ps
	$(PS2PDF) $@.ps manuscript.pdf

d7_double: create_dep_files create_dep_dirs d7_double.tex
	@echo "   .................................."
	@echo "   ---| Running target d7_double |---"
	@echo "   ##################################"
	@$(TEX) $@
	@echo "   ........................"
	@echo "   ---| Running $(BIB) |---"
	@echo "   ########################"
	@$(BIB) $@
	@echo "   ............................."
	@echo "   ---| Running final $(TEX) |---"
	@echo "   #############################"
	@$(TEX) $@
	@echo "   ......................."
	@echo "   ---| Running $(DVIPS) |---"
	@echo "   #######################"
	$(DVIPS) $(DVIPS_OPTS) < $@.dvi > $@.ps
	$(PS2PDF) $@.ps double.pdf

clean:
	-rm -f d7.aux d7.bbl d7.blg d7.dvi d7.ps d7.pdf
		
numbers: numbers.tex
	@$(TEX) $@
	$(DVIPS) $(DVIPS_OPTS) < $@.dvi > $@.ps
	$(PS2PDF) $@.ps $@.pdf

$(notdir $(DEP_FILES)):
	ln -f -s $(filter %$@,$(DEP_FILES)) $@

create_dep_files: $(notdir $(DEP_FILES))

$(notdir $(DEP_DIRS)):
	ln -f -s $(filter %/$@,$(DEP_DIRS)) $@

create_dep_dirs: $(notdir $(DEP_DIRS)) 
	


==> iter_thres.tex <==


% 2nd para
%%%

The separation of the deconvolution and denoising subproblems can be achieved through the use of the Expectation-Maximization (EM) algorithm in obtaining the MPL estimate. This was noted in~\cite{figueiredo03, daubechies04} under the model given by (\ref{eqn:gaussian:obs_familiar}). The class of MPL estimates includes the class of all possible MAP estimates. The latter is constrained in the type of penalty function that can be used, viz., it must be a valid p.d.f. On the other hand, the penalty function associated with a MPL estimate can be an arbitrary function.
%
Consider finding the MPL estimate
%
% eqn
%
\begin{equation}
\hat{\vtor\theta} = \text{argmax}_{\vtor\theta}
	( \log p(\vtor y|\vtor \theta) - \text{pen}(\vtor\theta,\vtor\phi) ),
\label{eqn:map_mple:est2}
\end{equation}
%
where $\vtor\phi$ is a vector of regularization parameters. 

% 3rd para
%%%

Select $\vtor z = \vtor\theta + \alpha \vtor{w}_1$ to be the \emph{complete data}, where $\vtor{w}_1 \sim \mathcal{N}(\vtor{w}_1;\vtor 0,\alpha^2\mathbf{I})$. As a result, one has the decomposition
%
% eqn
%
\begin{align}
\vtor z & = \vtor \theta + \vtor{w}_1 \nonumber \\
\vtor y & = \mathbf{H} \vtor z + \vtor{w}_2 
	\label{eqn:gaussian:decomp}
\end{align}
%
The noise $\vtor{w}_2 \sim \mathcal{N}(\vtor{w}_2;\vtor 0,\sigma^2\mathbf{I} - \alpha^2\mathbf{H}\mathbf{H}^T)$. Note that $\vtor{w}_1$ is AWGN, but $\vtor{w}_2$ is colored Gaussian noise. 
%
Define the spectral radius $\rho(\mathbf{A}) \triangleq \max_i |\lambda_i(\mathbf{A})|$, where $\lambda_i(\mathbf{A})$ are the eigenvalues of the square matrix $\mathbf{A}$. Decomposition (\ref{eqn:gaussian:decomp}) only works if $(\alpha/\sigma)^2 \le \rho(\mathbf{H}\mathbf{H}^T)^{-1}$. A visualization of the decomposition is given in Fig.~\ref{fig:gaussian_decomp}.
%
% fig
%
\begin{figure}[!h]
	\centering
	\resizebox{\FigOneSize}{!}{%
	\input{em_sep_c.pstex_t}}
	\caption{Decomposition of the deconvolution and denoising steps for Gaussian statistics.}
	\label{fig:gaussian_decomp}
\end{figure}

% 4th para
%%%

Denote by $\hat{\vtor z}^{(n)}$ and $\hat{\vtor\theta}^{(n)}$ the estimates of $\vtor z$ and $\vtor\theta$ in the $n$th EM iteration. They are obtained via the iterations
%
% eqn
%
\begin{align}
\hat{\vtor z}^{(n)} 
	& = \hat{\vtor\theta}^{(n-1)} + \left(\frac{\alpha}{\sigma}\right)^2 \mathbf{H}^T ( \vtor y - \mathbf{H}\hat{\vtor\theta}^{(n-1)} ) \text{ and }
	\label{eqn:gaussian:em_1}  \\
\hat{\vtor\theta}^{(n)} 
	& = \text{argmax}_{\vtor\theta} \left[
	-\frac{1}{2\alpha^2} \|\vtor\theta-\hat{\vtor z}^{(n)}\|^2 - \text{pen}(\vtor\theta,\vtor\phi)
	\right].
	\label{eqn:gaussian:em_2}
\end{align}
%
%
In this paper, the norm $\|\cdot\|$ without a subscript indicates the $l_2$ norm. 
%
Note that (\ref{eqn:gaussian:em_1}) is a Landweber iteration; consequently, it can be regarded as the deconvolution step. Likewise, the optimization (\ref{eqn:gaussian:em_2}) can be seen as the denoising step.
%
Equations (\ref{eqn:gaussian:em_1}) and (\ref{eqn:gaussian:em_2}) can be succinctly written as
%
% eqn
%
\begin{equation}
\hat{\vtor\theta}^{(n+1)} = \mathcal{D}\left(
	\hat{\vtor\theta}^{(n)} + c\mathbf{H}^T(\vtor y-\mathbf{H}\hat{\vtor\theta}^{(n)})\right),
\label{eqn:gaussian:em_succinct}
\end{equation}
%
where $\mathcal{D}(\cdot)$ is a denoising operation that depends on the form of $\text{pen}(\cdot,\vtor\phi)$, and $c = (\alpha/\sigma)^2$. 

Consider the class of denoising operators given by
%
% eqn
%
\begin{equation}
\mathcal{D}_T(\vtor x) \triangleq \sum_i T(x_i)\vtor e_i
\label{eqn:denoising_thres}
\end{equation}
%
for some $T:\mathbb{R}\rightarrow\mathbb{R}$, and the $\vtor e_i$s are the standard unit norm basis vectors in $\mathbb{R}^M$. $\mathcal{D}$ belongs to this class if the optimization (\ref{eqn:gaussian:em_2}) can be decomposed into $M$ identical optimizations for each $\theta_i$, $i=1,\ldots,M$. 
%
An example would be the LASSO estimator, where $\vtor\phi=(\beta)^T$ and $\text{pen}(\vtor\theta,\vtor\phi)=\beta\|\vtor\theta\|_1$. This results in $\mathcal{D}(\cdot)$ being of the form (\ref{eqn:denoising_thres}) with $T(x)=T_\text{s}(x;\beta/2)$, where $T_\text{s}(x;t)\triangleq (x-\text{sgn}(x)t)I(|x|>t)$ is the soft thresholding rule. 
%In general, $T(\cdot)$ will depend on $\text{pen}(\cdot,\vtor\phi)$. 

% 6th para
%%%

Conversely, given a denoising operator $\mathcal{D}_T(\cdot)$ in the iterative thresholding framework (\ref{eqn:gaussian:em_succinct}), what is the corresponding penalty term in the MPL framework? 
%
As this work concerns sparse reconstruction, we shall restrict $T(\cdot)$ to be a \emph{thresholding rule}~\cite{johnstone04} with certain additional properties. In particular, consider only thresholding rules $T(\cdot)$ with the property that $T(\cdot)$ is strictly increasing outside of $(-t,t)$. Consequently, $T(\cdot)$ is bijective on $\mathbb{R} \setminus (-t,t)$. With abuse of notation, let $T^{-1}(\cdot)$ denote the ``inverse'' of $T(\cdot)$, which will be discontinuous at $0$. 

\begin{prop} \label{prop:ebd_la:4} 
%-------------------------------------------------------------------------------
%
Suppose that $\|\mathbf{H}\| < 1$, and that the hyperparameter $\vtor\phi$ is fixed to $\vtor\phi^0$, i.e., a fixed thresholding rule $T(\cdot)=T(\cdot;\vtor\phi^0)$ is used. Assume that the thresholding rule $T(\cdot)$ satisfies the additional properties previously mentioned. 
%
The iterations (\ref{eqn:gaussian:em_succinct}) with $c=1$ and $\mathcal{D}(\cdot)=\mathcal{D}_T(\cdot)$ decrease the convex cost function $\Psi(\vtor\theta)$ in a monotonic fashion, where $\Psi(\vtor\theta)$ is given by
%
% eqn
%
\begin{align}
\Psi(\vtor\theta) & = \|\mathbf{H}\vtor\theta - \vtor y\|^2 + J(\vtor\theta)
\text{ where } J(\vtor\theta) \triangleq \sum_{i=1}^M J_1(\theta_i),
	\nonumber \\
\text{ and: } J_1(x) & \triangleq 2 T^{-1}(x)x - x^2 - 2 \int T(\xi) d\xi \bigg\vert_{\xi=T^{-1}(x)} 
	\label{eqn:em_ebd_la:4_1}
\end{align}
%
We use surrogate functions to reverse engineer the function $\Psi(\vtor\theta)$. Its usage here is inspired by~\cite{daubechies04}. For details of the derivation, refer to~\cite{tingthesis}. 
\end{prop} 
%-------------------------------------------------------------------------------

Notice that $J_1^\prime(x) = 2( T^{-1}(x) - x )$. A thresholding rule $T(x)$ is anti-symmetric and satisfies $0 \le T(x) \le x$ for all $x \ge 0$. Therefore, $J_1^\prime(x) \ge 0$ for $x>0$ and $J_1^\prime(x) \le 0$ for $x<0$. So $J(\vtor\theta)$ is convex; since $\|\mathbf{H}\vtor\theta-\vtor y\|^2$ is also convex, $\Psi(\vtor \theta)$ is convex as well. 

An intuitive understanding can be gained by computing the gradient of $\Psi$.
%
% eqn
%
%\begin{equation}
%\nabla \Psi(\vtor\theta) = 2 \mathbf{H}^T \mathbf{H} \vtor\theta - 2 \mathbf{H}^T \vtor y + 
%	2 ( T^{-1}(\theta_1)-\theta_1,\ldots, T^{-1}(\theta_M)-\theta_M )^T
%	\label{eqn:em_ebd_la:4_2}
%\end{equation}
%
%and so
%
% eqn
%
Then, $\nabla \Psi(\vtor\theta) = \vtor 0$ iff
\begin{equation}
%	& \iff \mathbf{H}^T \mathbf{H} \vtor\theta - \mathbf{H}^T \vtor y + (T^{-1}(\theta_1),\ldots,T^{-1}(\theta_M))^T - \vtor\theta = \vtor 0
%	\nonumber \\
%	& \iff T^{-1}(\theta_i) = \theta_i + (\mathbf{H}^T(y-\mathbf{H}\theta))_i, \; 1 \le i \le M
%	\nonumber \\
	\theta_i = T\left( \theta_i + (\mathbf{H}^T(y-\mathbf{H}\theta))_i \right), \; 1 \le i \le M
	\label{eqn:em_ebd_la:4_3} 
\end{equation}
%
A stationary point of $\Psi(\vtor\theta)$ is therefore a fixed point of the function
%
% eqn
%
\begin{equation}
m(\vtor\theta) \triangleq \sum_{i=1}^M T\left[ (\vtor\theta+\mathbf{H}^T(\vtor y-\mathbf{H}\vtor\theta))_i \right] \vtor{e}_i
	\label{eqn:em_ebd_la:4_4}
\end{equation}
%
The function $m$ above corresponds to one step of the iteration (\ref{eqn:gaussian:em_succinct}), i.e., the iterations are $\hat{\vtor\theta}^{(n+1)} = m(\hat{\vtor\theta}^{(n)})$. Consequently, the stationary points of $\Psi(\vtor\theta)$ are the fixed points of the iteration (\ref{eqn:gaussian:em_succinct}). 

\begin{list}{\textbf{Remark \arabic{ListCount}}}{\usecounter{ListCount}}

\item The following are true: (i) the iteration map $m$ is continuous with $\Psi(\vtor\theta) \ge \Psi(m(\vtor\theta))$, where equality holds iff $\vtor\theta$ is a fixed point of $m$ and (ii) the stationary points of $\Psi(\vtor\theta)$ are fixed points of the iteration ${\vtor\theta}^{(n+1)} = m({\vtor\theta}^{(n)})$. Therefore, any limit point of the sequence generated by ${\vtor\theta}^{(n+1)} = m({\vtor\theta}^{(n)})$ is a stationary point of $\Psi(\vtor\theta)$~\cite{lange00}.

\item If the columns of $\mathbf{H}$ are linearly independent, then $\|\mathbf{H}\vtor\theta-\vtor y\|^2$ is strictly convex, which makes the cost function $\Psi(\vtor\theta)$ strictly convex as well. In this case, the minimizer of $\Psi(\vtor\theta)$ is unique. In Remark 1, we noted that the sequence ${\vtor\theta}^{(n)}$ generated by $m$ converged to a minimizer of $\Psi(\vtor\theta)$. There, however, we did not have uniqueness. Under the condition of linear independence of the columns of $\mathbf{H}$, the minimizer is unique.

\item Proposition \ref{prop:ebd_la:4} enables us to \emph{design} a sparse prior or penalty by first specifying a good thresholding rule, e.g., those that possess oracular properties~\cite{antoniadis01}. Then, the iterative optimization of alternating Landweber and thresholding steps minimizes the cost function $\Psi(\vtor\theta)$ given by (\ref{eqn:em_ebd_la:4_1}). 
%This is illustrated in Fig.~\ref{fig:pen_design}. 
Once $\Psi(\vtor\theta)$ is available, any other optimization method can be used to find a minimizer. In particular, if there is a more efficient optimization method, or if there is a closed-form solution, that should be used.
%
% fig
%
%\begin{figure}[!h]
%	\centering
%	\input{design_pen.pstex_t}
%	\caption{Design of a sparse prior/penalty}
%	\label{fig:pen_design}
%\end{figure}

\end{list}




==> lit_review.tex <==

%
%>>> PAR 1
%

A plethora of results have appeared regarding problem (\ref{eqn:gaussian:obs_familiar}), both in the noiseless case when $\sigma=0$ and in the noisy case when $\sigma>0$. The review provided in this section does not aim to be exhaustive; rather, its purpose is to provide the reader with a background in which to frame the contribution of this paper. 
%The noisy case is reviewed in more detail, as it is the focus of this work.

% MT: why are we talking about the noiseless case??

\subsection{Noiseless case}

%
%>>> PAR 2
%
In the noiseless case, i.e., $\sigma=0$, (\ref{eqn:gaussian:obs_familiar}) reduces to finding the sparsest representation of $\vtor y$ in terms of the column of $\mathbf{H}$, i.e.,
%
% eqn
%
\begin{equation}
P_0: \text{ minimize } \|\vtor\theta\|_0 \text{ such that } \vtor y = \mathbf{H}\vtor\theta
	\label{eqn:sparse_problem:P0}
\end{equation}
%
where the $l_0$ counting measure is defined as $\|\vtor x\|_0 \triangleq \#\{i: x_i \neq 0\}$. The general solution of (\ref{eqn:sparse_problem:P0}) requires an enumerative approach, resulting in a search that is exponential in $M$. This is impractical for large images. If the columns of $\mathbf{H}$ are sufficiently uncorrelated \emph{and} $\vtor\theta$ sufficiently sparse, the solution to P0 is unique; moreover, P0 can be solved via orthogonal matching pursuit (OMP) or basis pursuit (BP)~\cite{tropp04}. Other techniques are also possible. Prior work on this problem includes~\cite{mallat93,gorodnitsky97,chen99,gribonval03}. Using the terminology in~\cite{tropp04}, define the \emph{coherence} of $\mathbf{H}$ as
%
% eqn
%
\begin{equation}
\mu \triangleq \max_{i \neq j} |\langle \vtor h_i, \vtor h_j \rangle|.
	\label{eqn:coherence}
\end{equation}
%
The coherence is the largest pairwise correlation between distinct columns of $\mathbf{H}$. Let $\Omega \triangleq \{1,\ldots,M\}$ be the column index set of $\mathbf{H}$. A more general notion of coherence is the \emph{cumulative coherence} function $\mu_1(m)$, defined as
%
% eqn
%
\begin{equation}
\mu_1(m) \triangleq 
	\max_{|\Lambda|=m} 
	\max_{\{\vtor h_i: i \notin \Lambda\}}
	\sum_{j \in \Lambda} |\langle \vtor h_i, \vtor h_j \rangle|,
	\label{eqn:cum_coherence_fn}
\end{equation}
%
where $\Lambda \subseteq \Omega$. Let $\Lambda(\vtor x) \triangleq \{ i : x_i \neq 0 \}$. If it is known that $|\Lambda(\vtor\theta)| \le m$, the criterion needed to ensure reconstruction of $\vtor\theta$ via OMP or BP is given by~\cite[Thm.~B]{tropp04}, which is $\mu_1(m-1)+\mu_1(m)<1$. A more restrictive but intuitive condition is 
%
% eqn
%
\begin{equation} \label{eqn:erc_noiseless}
m < \frac{\mu^{-1}+1}{2}
\end{equation}
%
As $m$ increases, the columns of $\mathbf{H}$ must be more uncorrelated in order to achieve exact reconstruction. If $\mathbf{H}$ is a correlation matrix--and thus each of its columns have high (pairwise) correlation with another column--the maximal $m$ that satisfies~\cite[Thm.~B]{tropp04} is greatly limited. 

\subsection{Noisy case}

%
%>>> PAR 3
%

A problem related to (\ref{eqn:gaussian:obs_familiar}) is when $\vtor w$ is not a statistical quantity, but is rather bounded in some fashion, e.g., in $l_2$ norm, an element-wise bound, etc. The CLEAN algorithm~\cite{hogbom74}, used to restore star field images, minimizes the $l_1$ norm of $\vtor\theta$ subject to $|\nu_i|\le\epsilon_i$ and $\theta_i \ge 0$, where $\vtor\nu \triangleq \mathbf{H}\vtor\theta-\vtor y$ and $\epsilon_i \ge 0$~\cite{marsh87}. Use of the $l_p, 0 < p < 1$ quasi-norm is considered in~\cite{jeffs93}.

%
%>>> PAR 4
%

To our knowledge, the noisy case of (\ref{eqn:gaussian:obs_familiar}), i.e., $\sigma>0$, was first considered in~\cite{alliney94}. Suppose that there exists a prior $p(\vtor\theta|\vtor\zeta)$ on $\vtor\theta$, where $\vtor\zeta$ denotes the vector of \emph{hyperparameter(s)}. In~\cite{alliney94}, the authors consider Gaussian and Laplacian priors for $p(\vtor\theta|\vtor\zeta)$, and propose using the MAP estimate for $\hat{\vtor\theta}$, When the latter prior is used in a MAP framework, the resulting $\hat{\vtor\theta}$ is the maximum penalized likelihood estimate (MPLE) with a $l_1$ norm penalty. 

%
%>>> PAR 5
%

The case when $p(\vtor\theta|\vtor\zeta)=\prod_n p(\theta_n|\zeta_n)$ such that $p(\theta_n|\zeta_n) \sim \mathcal{N}(0,\zeta_n)$ was given the moniker Sparse Bayesian Learning (SBL) in~\cite{tipping01}. Necessarily, $\zeta_n \ge 0$ for each $n=1,\ldots,N$. When $\sigma=0$, the $\vtor\zeta$ that produces a maximally sparse $\vtor\theta$ achieves the global minimum of the MML cost function~\cite[Thm.~1]{wipf04}. However, the global minimum is not unique, and multiple local minima potentially exist. When $\sigma>0$, one is only assured that the resulting $\hat{\vtor\theta}$ will satisfy $\|\hat{\vtor\theta}\|_0<N$~\cite[Thm.~2]{wipf04}. For $N=M$, an estimate $\hat{\vtor\theta}$ that satisfies this condition is not necessarily sparse: most $\vtor\theta \in \mathbb{R}^N$ would satisfy $\|\vtor\theta\|_0<N$. A detraction of using SBL is its high computational cost due to the expectation-maximization (EM) iterations used to obtain $\hat{\vtor\zeta}$. In each E-step, the inversion of a $\min(M,N) \times \min(M,N)$ matrix is required. While an alternative iteration leads to faster convergence in an empirical study, convergence to a local minimum is not assured~\cite[(44)]{tipping01}. In any event, a matrix inversion is still present in each iteration.

%
%>>> PAR 6
%

The estimator formed when a Laplacian prior is used for $p(\vtor\theta|\vtor\zeta)$ has been popularized in~\cite{tibshirani96} as the lasso. It is given by
%
% eqn
%
\begin{equation} \label{eqn:lasso}
\hat{\vtor\theta} = \mathop{\text{argmin}}_{\vtor\theta} \{ \|\mathbf{H}\vtor\theta - \vtor y\|_2^2 + \zeta_1 \|\vtor\theta\|_1 \}.
\end{equation}
%
The lasso also know by others as BP denoising~\cite{chen99}. The lasso has been shown to have good properties when $\|\vtor w\|_2$ is bounded by a known constant, e.g.,~\cite[Thm.~4]{fuchs05},~\cite[Thm.~1]{candes05},~\cite[Thm.~3.1]{donoho06}, and~\cite[Corr.~8]{tropp06}. The first and last results previously mentioned make use of $\mu |\Lambda(\vtor\theta)| < 1/2$, which is similar to condition (\ref{eqn:erc_noiseless}). The second result makes use of the notion of an S-restricted isometry constant $\delta_S$: see~\cite{candes05} for further details. A necessary condition for the third result is the condition $|\Lambda(\vtor\theta)| < (\mu^{-1}+1)/4$. Note that the problem addressed in this work, viz., (\ref{eqn:gaussian:obs_familiar}), does not have bounded $\|\vtor w\|_2$. Nonetheless, one can derive a probability of success of the lasso along the lines of~\cite[Sec.~IV.D]{tropp06}. 

The lasso is not the only method that has been investigated to solve the sparse problem in the presence of noise. The equality constraint in $P_0$ can be relaxed to get
%
% eqn
%
\begin{equation} \label{eqn:sparse_problem:P0delta}
P_{0,\delta}: \text{ minimize } \|\vtor\theta\|_0 \text{ such that } 
	\|\vtor y - \mathbf{H}\vtor\theta\|_2 \le \delta
\end{equation}
%
for some $\delta > 0$. Let $\hat{\vtor\theta}_{0,\delta}$ denote the solution to $P_{0,\delta}$. When (\ref{eqn:erc_noiseless}) is satisfied for $m = |\Lambda(\vtor \theta)|$, $\|\hat{\vtor\theta}_{0,\delta}-\theta\|_2$ is upper-bounded~\cite[Thm.~2.1]{donoho06}. Yet another alternative is StOMP, an extension of OMP~\cite{donoho06_stomp}. While the noise term $\vtor w$ is not explicitly taken into account, its effect is incorporated by assuming that the columns of $\mathbf{H}$ come from a specific random distribution, e.g., the uniform spherical ensemble (USE), or the uniform random projection ensemble (URPE). Under the USE distribution, $\vtor h_i$ are i.i.d.~points of the unit sphere $S_N(0) \triangleq \{ \vtor x \in \mathbb{R}^N: \|\vtor x\|_2 = 1\}$. Under the URPE distribution, $\vtor h_i$ are the first $N$ rows of a $M \times M$ random orthogonal matrix, where it is assumed that $N < M$. See~\cite{donoho06_stomp} for further details. A third approach previously taken is maximum entropy (ME) reconstruction, which is the MPLE with the entropy of $\vtor\theta$ taken as the penalty (regularizing) term~\cite{burch83}. While a ME estimate will have strictly positive values, this is not necessarily an impediment to deconvolving a sparse image from a noisy measurement. Suppose that $\vtor\theta$ is sparse, and that its non-zero elements are all strictly positive. The image $c \vtor 1 + \vtor\theta$ for $c>0$ will also look visually sparse. Unlike the problems of atomic decomposition or subset selection, one of the most important criterion of an image reconstruction is how \emph{visually similar} the estimate is to the original. 
%When applied to the sparse denoising problem, viz., the problem considered in this paper but with $\mathbf{H}=\mathbf{I}$, the lasso has better worst case performance than ME~\cite{donoho92}.
When there are positive and negative $\theta_i$, the range of values in the ME estimate that should be interpreted as ``empty space'' has to be determined.

The stability and support results of the lasso or $P_{0,\delta}$ solution mentioned above all require that
%
% eqn
%
\begin{equation} \label{eqn:erc_approx_general}
\mu |\Lambda(\vtor\theta)| \lessapprox c
\end{equation}
%
where $c=1/2$ or $1/4$. For a given $\mathbf{H}$, this condition imposes a maximum value on the support size of $\vtor\theta$ such that some statement of optimality can be said. The previous works typically focused on the case where the columns of $\mathbf{H}$, either taken in a pairwise or subset-wise fashion, have low correlation, e.g., union of orthonormal bases. As such, (\ref{eqn:erc_approx_general}) is not too restrictive, since one would expect $\mu$ to be generally ``small''. However, if $\mathbf{H}$ is a convolution matrix, then $\mu$ is larger. In the simulation section later on in this work, one example uses a convolution matrix $\mathbf{H}$ where $\mu \approx 0.86089$. Substituting this in to (\ref{eqn:erc_approx_general}) requires that $|\Lambda(\vtor\theta)| \lessapprox c/0.86089 < 1$ for $c=1/2$ or $1/4$.

If $\vtor w$ or a bound on its norm are known, tests for the optimality of $\hat{\vtor\theta}$ are available, regardless of how $\hat{\vtor\theta}$ is obtained~\cite{gribonval06_eurasip}. 

\subsection{Choice of hyperparameter}

The algorithms mentioned thus far depend on additional parameters that are referred to in this work as hyperparameters, e.g., $\vtor\zeta$ in the prior $p(\vtor\theta|\vtor\zeta)$ or $\vtor\epsilon$ in CLEAN. They are also referred to as \emph{regularization} or \emph{tuning} parameters. If (\ref{eqn:erc_approx_general}) is satisfied for the proper $c$, the stability and support results in~\cite{fuchs05,candes05,donoho06,tropp06} offer guidance as to how to select the lasso hyperparameter. Results that require knowledge of $\Lambda(\vtor\theta)$ are not applicable, however, as this a priori information is not known. In the case when (\ref{eqn:erc_approx_general}) is \emph{not} satisfied, the body of work~\cite{fuchs05,candes05,donoho06,tropp06} does not point to an optimal value of the hyperparameter to use.

Let us enumerate methods that have been used to estimate the hyperparameter(s). These are generally applicable when when one is working with a hierarchical model. In~\cite{alliney94}, MML is used. While the MML $p(\vtor y|\vtor \zeta)$ can be evaluated in closed-form for the Gaussian prior~\cite[(A1.8)]{alliney94}, approximations are required when the prior is Laplacian: see~\cite[(A2.3)]{alliney94} and~\cite[(A3.6)]{alliney94}. In~\cite{tibshirani96}, three methods are used to estimate lasso's hyperparameter: CV, GCV, and SURE. An orthonormal $\mathbf{H}$ is assumed in the derivation of the SURE estimate.

\subsection{Other priors for the sparse image}

Recall that a Bayesian perspective of lasso is that of the MAP estimate with an i.i.d.~Laplacian prior on $\vtor\theta$. The lasso hyperparameter is directly related to the scale parameter in the Laplacian p.d.f. While the lasso---and thus the Laplacian prior---has strong optimality properties, consider the experiment where one draws  $M$ i.i.d.~samples from a Laplacian distribution. The expected number of samples that are exactly zero is zero, as the Laplacian c.d.f.~is continuous. This discordant result suggests the incorporation of a discontinuity at zero. Indeed, in~\cite{johnstone98}, the following sparse prior is used
%
% eqn
%
\begin{equation} \label{eqn:gaze}
p(\theta_i) = (1-w) \delta(\theta_i) + w g(\theta_i;0,\nu^2),
\end{equation}
%
where $\delta(\cdot)$ is the Dirac delta function, $0 \le w \le 1$, and $g(\cdot;a,b^2)$ is a Gaussian p.d.f.~with mean $a$ and variance $b^2$. Later work by the same authors involve use of the LAZE p.d.f.~\cite{johnstone04}, i.e.,
%
% eqn
%
\begin{equation} \label{eqn:laze}
p(\theta_i) = (1-w) \delta(\theta_i) + w \gamma(\theta_i;a),
\end{equation}
%
where $\gamma(x;a)=(1/2)ae^{-a|x|}$ is the Laplacian p.d.f. 
%The hyperparameter vector $\vtor\zeta=(a,w)$ for the LAZE prior. 
The work~\cite{johnstone04} studies the sparse denoising problem, viz., the problem considered in this paper but with $\mathbf{H}=\mathbf{I}$. A general class of heavy-tailed $\gamma$--which includes the Laplacian p.d.f.--is considered. With the risk measured by the $q$th power loss for $0 < q \le 2$., the method proposed in~\cite{johnstone04} asymptotically attains the optimal minimax risk over a wide range of sparse signal classes. The LAZE prior is intuitive: the proportion of non-zero elements in $\vtor\theta$ is, on average, $w$. Given $M$ i.i.d.~samples from (\ref{eqn:laze}), the expected number of values that equal zero is $Mw$. The Laplacian p.d.f.~is a special case of the LAZE p.d.f.~with $w=1$. We note that the LAZE p.d.f.~is both a sparse \emph{and} heavy-tailed prior.

\subsection{Implementation approaches} \label{sec:lit_review:impl}

The lasso can be solved via iterated thresholding operations~\cite{figueiredo03}. Specifically, EM can be applied using $\vtor z = \vtor \theta + \alpha \vtor w_1$ as the \emph{complete data}, where $\vtor w_1 \sim \mathcal{N}(0,\alpha^2\mathbf{I})$ and $\alpha \le \sigma/\|\mathbf{H}\|_2$. Denote by $\vtor{\hat{\theta}}^{(n)}$ the estimate in the $n$th EM iteration. Let $\vtor e_i \in \mathbb{R}^M$ denote the standard unit vectors. For $\vtor x \in \mathbb{R}^M$, $S_{T_s,t}(\vtor x) \triangleq \sum_i T_s(x_i;t) \vtor e_i$ applies the soft thresholding rule $T_s(x;t) = (x-\text{sgn}(x)t)I(|x|>t)$ to each element of $\vtor x$. The EM iterations can be expressed as
%
% eqn
%
\begin{equation} \label{eqn:em_iter:lasso}
 \vtor{\hat{\theta}}^{(n+1)} = S_{T_s,\zeta/2} \left( \vtor{\hat{\theta}}^{(n)} +
	(\alpha/\sigma)^2 \mathbf{H}^\prime ( \vtor y - \mathbf{H} \vtor{\hat{\theta}}^{(n)} \right).
\end{equation}
%
The expression within the argument of $S_{T_s,\zeta/2}(\cdot)$ is a Landweber iteration. The work of~\cite{daubechies04} considers an $l_p$ penalty on $\vtor\theta$ for $1 \le p \le 2$, and iterative thresholding operations similar to (\ref{eqn:em_iter:lasso}) are derived. Convergence results are given in~\cite{daubechies04}. The least angle regression (LARS) algorithm can be used to implement the lasso~\cite{efron04}. LARS iterates over the support of $\vtor{\hat{\theta}}$: in each iteration, the lasso estimate is exactly computed. LARS has lower complexity and does not suffer from precision issues, which would be the case in the iterative approach if one did not take a sufficiently large number of iterates. On the other hand, LARS requires that the columns of $\mathbf{H}$ be linearly independent; this is not required by the iterative approach. The selection of individual columns of $\mathbf{H}$ is also needed for LARS. In the simulation study of this paper, however, we show that this is not an obstacle for a relatively large problem.


==> sim_img3_tip.tex <==

% 1st para
%%%

The quality of the hyperparameter estimates of MAP1 and MAP2 is examined when applied to the LAZE image. The mean hyperparameter estimate $\hat{\vtor\phi}=(\hat{a},\hat{w})$ is plotted vs.~SNR in Figs.~\ref{fig:sim:hyp}a--b. For MAP2, two values of $g^\ast$ are used: $2^{-1/2}$ and $10^3$.
%
% fig
%
\begin{figure}[htb]
%
\begin{minipage}[b]{.48\linewidth}
	\centering
	\centerline{\epsfig{figure=tip_hyp07/ahat,width=\FigSevenSize}}
	\vspace{0.25cm}
	\centerline{(a) $\hat{a}$}
\end{minipage}
%
\begin{minipage}[b]{0.48\linewidth}
	\centering
	\centerline{\epsfig{figure=tip_hyp07/what,width=\FigSevenSize}}
	\vspace{0.25cm}
	\centerline{(b) $\hat{w}$}
\end{minipage}
%
\caption{Hyperparameter estimate vs.~SNR for MAP1 and MAP2 with $g^\ast=2^{-1/2}, 10^3$.}
\label{fig:sim:hyp}
%
\end{figure}
%
MAP1's $\hat{a}$ appears to converge as the SNR increases, whereas MAP2's estimates slowly increase with higher SNR. However, MAP1's estimate is far from the true value of 1, whereas MAP2's estimates are closer. For both values of $g^\ast$, MAP2's $\hat{a}$ is close to 1 when the SNR is in the range of 2--8 dB. Consider next $\hat{w}$ in Fig.~\ref{fig:sim:hyp}b. For the MAP-based methods, $\hat{w}$ increases with higher SNR. When the SNR is in the range of 2--8 dB, the estimates are close to $0.026$, which is the true value. 

% 2nd para
%%%

The $E_d$ error curves of MAP1 and the two MAP2 estimators are illustrated in Fig.~\ref{fig:sim:laz_ed}. In addition, the LASSO-SURE error curve is displayed as a basis of comparison.
%
% fig
%
\begin{figure}[htb]
	\centering
	\epsfig{figure=tip_hyp07/ed_map2,width=\FigEightSize}
	\caption{$E_d$ error curves for MAP1, MAP2, and LASSO-SURE with the LAZE image.}
	\label{fig:sim:laz_ed}
\end{figure}
%
When the hyperparameter estimate is relatively unbiased, i.e., SNR $\approx$ 2--8 dB, we expect the MAP methods to perform well under the $E_d$ criterion. This is because MAP minimizes the error probability $P_e(\hat{\vtor\theta})=P(\|\vtor\theta-\hat{\vtor\theta}\|>\epsilon)$, and the $E_d(\vtor\theta,\hat{\vtor\theta})$ criterion can be regarded as the error probability on the support of $\vtor\theta$. 

% 3rd para
%%%

Indeed, when the SNR is in the range of 2--8 dB, which is where the hyperparameter estimates are relatively unbiased, the MAP methods have lower $E_d$ curves than LASSO-SURE. The increase of MAP2's $E_d$ curve when $g^\ast=2^{-1/2}$ closely parallels the increase of its $\hat{w}$. Interestingly enough, the bias of $\hat{a}$ of MAP1 does not result in poor performance in terms of $E_d$. Since MAP1's $\hat{w}\le 1/2$, the hybrid thresholding rule is used in (\ref{eqn:map1:theta}). In the simulation, $\alpha<1$, and because $\hat{w}$ is small over the range of SNRs considered, the expression for $t_1 = \hat{a}\alpha^2 + \sqrt{2\alpha^2\log((1-\hat{w})/\hat{w})}$ is dominated by the second term.




